A Core Model for Choreographic Programming

Choreographic Programming is a programming paradigm for building concurrent programs that are deadlock-free by construction, as a result of programming communications declaratively and then synthesising process implementations automatically. Despite strong interest on choreographies, a foundational model that explains which computations can be performed with the hallmark constructs of choreographies is still missing. In this work, we introduce Core Choreographies (CC), a model that includes only the core primitives of choreographic programming. Every computable function can be implemented as a choreography in CC, from which we can synthesise a process implementation where independent computations run in parallel. We discuss the design of CC and argue that it constitutes a canonical model for choreographic programming.

==> chc_typing.tex <==
\begin{figure}
\begin{displaymath}
\scriptsize
\begin{array}{c}
\infer[\!\!\rname{T}{Com}]
{
	\tjudge{\Gamma;\Theta}{\scgencom;C}{\Delta, k: \gtcom{\role A}{\role B}{S}; G}
}
{
	\Gamma \seq e@\pid p: S
	\!&\!
	\Theta \seq \pid p: k[\role A], \pid q: k[\role B]
	\!&\!
	\tjudge{\Gamma,x@\pid q:S;\Theta}{C}{\Delta, k: G}
}
\\\\
\infer[\!\!\rname{T}{Sel}]
{
	\tjudge{\Gamma;\Theta}{\scgenselj;C}{\Delta, k: \gtgenbranch}
}
{
	\Theta \seq \pid p: k[\role A], \pid q: k[\role B]
	&
	j \in I
	&
	\tjudge{\Gamma;\Theta}{C}{\Delta, k: G_j}
}
\\\\
\infer[\!\!\rname{T}{Cond}]
{
	\tjudge{\Gamma;\Theta}{\scgencond}{\Delta}
}
{
	\tjudge{\Gamma;\Theta}{C_1}{\Delta}
	&
	\tjudge{\Gamma;\Theta}{C_2}{\Delta}
}
\end{array}
\end{displaymath}
\caption{Channel Choreographies, Typing Rules (selection).}
\label{fig:cc_typing_rules}
\end{figure}
% 

==> conclusions.tex <==
%!TEX root = main.tex
\reftwo[,inline]{6a}{critical analysis of the results}

We developed Core Choreographies (CC), a calculus which we argued can constitute a foundation for choreographic 
programming.
We motivated the primitives for CC by showing that they extend a minimal set necessary for Turing completeness by 
including only label selection, which is a characteristic feature of choreography calculi.
For completeness' sake, we showed how to encode label selections as value communications,
thus obtaining a smaller calculus of Minimal Choreographies (MC) that is still Turing complete.
% but discussed why the resulting 
% choreographies are not satisfactory.

The development of CC has already enabled us to study theoretical questions in choreographic programming in a minimal setting.
In~\cite{ourasyncstuff}, we showed that CC is unable to encode asynchronous communication, and discussed
which primitives to add in order to be able to mimic this behaviour in a synchronous semantics.
In~\cite{ourextractionstuff}, we considered the problems of (i) deciding
whether a process implementation can be described by a choreography, and (ii) extracting such a choreography 
in the affirmative case; we showed that, for CC and SP, both problems are solvable in exponential time.
Finally, in~\cite{ourPCstuff} we studied how to extend CC with general sequential composition -- a feature that is 
unavailable in most choreography calculi equipped with recursion -- together with other commonly occurring primitives 
that are useful in practice (process spawning and name passing).
The expressivity of the resulting calculus was demonstrated in~\cite{lcf:fm:16a}.

The results in Section~\ref{sec:translation} justify that it makes sense to use CC for these studies, in addition to 
the technical convenience of working in a setting that is as simple as possible.
Our study of encoding asynchronous communications~\cite{ourasyncstuff} again identifies a minimal set of primitives that 
must be present in a choreography language to build such an encoding, and the encoding itself can be structurally 
extended to most languages.
The results on extraction~\cite{ourextractionstuff} give us a lower bound for the complexity of deciding the same 
problem in other choreography calculi (since they all include CC), and identify some technical challenges that will 
always be present.
The work in~\cite{ourPCstuff} and~\cite{lcf:fm:16a}, on the other hand, illustrates how
concepts defined for CC (for example, the notion of ``running in parallel'', Definition~\ref{defn:parrun}) are naturally 
applicable in more complex settings.
%
% We presented Minimal Choreographies, MC, and showed that it is Turing complete and projectable to a
% process calculus, but by removing or simplifying any of its syntactic primitives one or both of those 
% properties break.
% MC is a sublanguage of Core Choreographies, CC, which include the extra primitive of label selection that is
% typical in other choreography calculi.
% While label selections are not essential for Turing completeness, they make projectability easier to ensure
% and amendment simpler to define -- two properties which justifies including them in a minimalist calculus.
% 
% The informed reader will recognise that our proof of Turing completeness for MC has a similar structure to that for 
% the URM.
% The proof is indeed more relevant for its consequences rather than its technical details.
% In particular, it guided us in the design of MC.
% The developments of previous choreography models were guided by the need for practical features which, albeit
% useful in practice, concealed the foundations of choreographic programming.
% The design of MC, CC, and our EPP, guided by the notion of computability, could thus be seen as our major
% technical contribution, since they show that choreographic programming has clear foundations when it comes to
% computation.
%
%% MC and CC provide us with a foundation to reason about the computational power of choreography languages, as
%% discussed in \S~\ref{sec:implications}.
%% It is thus a useful reference, due to its succint formulation and minimality.
%% From this point, 

Our results support the claim that there are substantial advantages to gain from first studying 
choreographic programming in itself, abstracting from features that are specific to other models (like channels in 
process calculi), and then applying the obtained insights to particular scenarios.
We believe that CC is a useful step in this direction, and that it will serve as a stepping stone for the future 
developments of the paradigm of choreographic programming in general.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

